A long-range memory stochastic model of the return in financial markets

We present a nonlinear stochastic differential equation (SDE) which mimics the probability density function (PDF) of the return and the power spectrum of the absolute return in financial markets. Absolute return as a measure of market volatility is considered in the proposed model as a long-range memory stochastic variable. The SDE is obtained from the analogy with earlier proposed model of trading activity in the financial markets and generalized within the nonextensive statistical mechanics framework. The proposed stochastic model generates time series of the return with two power law statistics, i.e., the PDF and the power spectral density, reproducing the empirical data for the one minute trading return in the NYSE.

==> CHANGES <==
Changes from elsart 2.19 to 2.20
================================

Enable \tableofcontents at the end of the frontmatter
Suppress linenumbering in the frontmatter
Correct an error in the \collab command
Define \@ptsize to report the point size
Add \endNoHyper to \endfrontmatter
Change \let to \def in \endfigure, \endtable and \endalgorithm commands

Changes from elsart 2.18 to 2.19
================================

2006-05-01: added narrowdisplay option
2006-05-01: added draft and final option
2006-05-01: added \ensuremath around \ell in \@alph (suggested by
			Alik Widge)
2006-05-01: added \cal and \mit as alternatives for \mathcal and
			\mathnormal
2006-05-01, in \collab@fmt: added check for the presence of a
			footnote symbol
2001-02-22, in \collab@arg: \first@collab has been replaced with
			\first@author
2001-02-22, in \ead@au: changed \edef to \def
2001-12-14, in \collapse@citex: added code to remove leading spaces
			on cite key, from ltbibl

Changed files July 2006
=======================

Updated: elsart.cls.

New: elsart1p.cls, elsart3p.cls, elsart5p.cls.

Removed: elsart.sty, elsart12.sty. These are outdated.

Rewritten: instructions-harv.pdf, instructions-num.pdf. These replace
model-harv.pdf and model-num.pdf.

Removed: instraut. These instructions are outdated.

Modified: template-harv.tex, template-num.tex. The lineno package was
added.

